Algorithmic Fairness Datasets: the Story so Far

Data-driven algorithms are studied in diverse domains to support critical decisions, directly impacting people's well-being. As a result, a growing community of researchers has been investigating the equity of existing algorithms and proposing novel ones, advancing the understanding of risks and opportunities of automated decision-making for historically disadvantaged populations. Progress in fair Machine Learning hinges on data, which can be appropriately used only if adequately documented. Unfortunately, the algorithmic fairness community suffers from a collective data documentation debt caused by a lack of information on specific resources (opacity) and scatteredness of available information (sparsity). In this work, we target data documentation debt by surveying over two hundred datasets employed in algorithmic fairness research, and producing standardized and searchable documentation for each of them. Moreover we rigorously identify the three most popular fairness datasets, namely Adult, COMPAS and German Credit, for which we compile in-depth documentation. This unifying documentation effort supports multiple contributions. Firstly, we summarize the merits and limitations of Adult, COMPAS and German Credit, adding to and unifying recent scholarship, calling into question their suitability as general-purpose fairness benchmarks. Secondly, we document and summarize hundreds of available alternatives, annotating their domain and supported fairness tasks, along with additional properties of interest for fairness researchers. Finally, we analyze these datasets from the perspective of five important data curation topics: anonymization, consent, inclusivity, sensitive attributes, and transparency. We discuss different approaches and levels of attention to these topics, making them tangible, and distill them into a set of best practices for the curation of novel resources.

==> misc.tex <==

\section{Intro}

Relevant work:
\begin{itemize}
    \item // OK // \citet{gebru2018datasheets} documentation proposal
    \item // OK // \citet{holland2018dataset} documentation proposal
    \item // OK // \citet{paullada2020data} concerns about dataset development and use (representativeness,  lack of rigorous and standardized dataset documentation) 
    \item // OK // \citet{prabhu2020large} emphasize need for better curation process and problems with ImageNet
    \item \citet{yang2020towards} biases and problems with ImageNet
    \item // OK // \citet{bender2018data} documentation proposal for NLP
    \item \citet{geiger2020garbage} call out disparate transparency in reporting where human-annotated labels come from.
    \item \cite{jo2020lessons} discuss important topics in data collection and areas where we could do better (inclusivity, consent, transparency)
    \item \citet{ekstrand2018privacy} mention de-anonymizatoin risks.
    \item // OK // \citet{miceli2021documenting} issues that hinder the documentation of image datasets
    \item // OK // \citet{garbin2021structured} datasheet for CheXpert 
    \item // OK // \citet{bandy2021addressing} datasheet for Book Corpus
    %\item \afabcomment{In the presentation for \cite{hutchinson2021towards} there are some interesting references. Also the paper itself is worth commenting.}
    \item \citet{bender2021:dangers} we should borrow the concept of documentation debt mentioned therein in relation to large datasets
    \item \citet{hardt2021facing} limitations of Adult
    \item \citet{gromping2019:sg} limitations of German
    \item \citet{barenstein2019propublica} problems with COMPAS
    \item //OK// increased attention to datasets in ML community: NeurIPS dedicated track and links to dartasets on arXiv  \url{https://medium.com/paperswithcode/datasets-on-arxiv-1a5a8f7bd104}  \url{https://neuripsconf.medium.com/announcing-the-neurips-2021-datasets-and-benchmarks-track-644e27c1e66c}
    \item documentation proposal \url{https://pair-code.github.io/datacardsplaybook/}
    \item //OK// \citep{denton2020bringing} contestation of benchmark datasets
    \item \citet{barocas2019fair} Analysis of pros and cons of benchmarks. They abstract away context so that practitioners need to domain expertise. Discuss roles of datasets. Against pubblish IFF SOTA. ``Using benchmark datasets to make generalizable claims about fairness requires careful attention to issues of context, sampling, and validity.''
    \item // OK // \citep{oneto2020fairness} list 24 datasets used in fair ML research.
    \item // OK // \citep{zehlike2021fairness} list 19 datasets used in fair ranking. ``The papers surveyed here rarely substantiate their choice of an experimental dataset, other than that by the fact that the dataset was available, and that items in it have scores on which to rank.''
\end{itemize}

Recent fairness research \citep{gebru2018datasheets,holland2018dataset,bender2018data,jo2020lessons,prabhu2020large} has been instrumental in making the broader machine learning community aware of the need for more attentive practices of dataset curation and documentation. Notable initiatives in this direction include a dedicated NeurIPS 2021 track\footnote{\url{https://neuripsconf.medium.com/announcing-the-neurips-2021-datasets-and-benchmarks-track-644e27c1e66c}} and arXiv initiative to support links to datasets.\footnote{\url{https://medium.com/paperswithcode/datasets-on-arxiv-1a5a8f7bd104}}

Some of these works have highlighted problems and limitations of specific datasets, such as ImageNet \citep{prabhu2020large,yang2020towards}. Some works contest the use of benchmark datasets in machine leanring in general \citep{denton2020bringing}, while others try to analyze both perks and downsides \citep{barocas2019fair}. A common criticism against large benchmark datasets is that they are often not properly documented \citep{bender2021:dangers}, but a lack of rigorous and standardized dataset documentation is general and important problem for dataset development and use in machine learning \citep{paullada2020data}.

Several documentation proposals have been brought forth, both generic \citep{gebru2018datasheets,holland2018dataset} and domain-specific \citep{bender2018data,miceli2021documenting}, which should help provide useful context and reduce the \textbf{opacity} of datasets. Following these proposals, a couple works of retrospective compilation of detailed documentation for single datasets have been undertaken  \citep{bandy2021addressing,garbin2021structured}, benefitting  the whole research community.

One additional issue with dataset documentation is its \textbf{scatteredness}. While relevant information exists for each dataset, it is not trivial to find. For example, an erratum for the poplar German credit dataset has been available since 2019 \citep{gromping2019:sg,gromping2019:sg2}, but few people seem to have taken notice. Perhaps more importantly, the mere fact that a given dataset exists and is relevant to a given task or a given domain may be unknown, especially for resources that are not particularly popular within a community \afabcomment{Qui linkare a un istogramma dell'utilizzo dei dataset da fare (pochi usati tantissimo, tanti usati pochissimo)}. Popular surveys of fairness in machine learning focus on fairness definitions, tasks and methods \citep{mehrabi2019survey,caton2020fairness}. A more recent survey work lists 24 fairness datasets \citep{oneto2020fairness}. Another recent survey focused on fair ranking lists and briefly describes 19 datasets that have been used for this task \citep{zehlike2021fairness}.

Arguably, both opacity and scatteredness have contributed to a documentation gap in the machine learning community. In this work, we help close this gap for the fair machine learning community. 


``Use of a dataset for empirical validation in a seminal paper often leads to follow-up work replicating those experiments and  establishing that dataset as a de facto benchmark for the problem studied. Expectations of the typical conference review process, which limit discussion and author rebuttal relative to journal publication norms of other fields, reinforce this positive feedback loop. Omitting a commonly-used dataset in an experiments section is a dangerous gamble for authors whose paper may be rejected for failing to compare to established benchmarks. Thus, researchers are incentivized to continuously replicate even flawed experiments. This is not a purely hypothetical concern: this compounding effect is one of the reasons for the (in our opinion) overuse of the COMPAS dataset'' \citep{bao2021COMPASlicated}


``Because existing datasets are not race-aware except RFW, we use our BUPT-Globalface and BUPTBalancedface datasets to train our models'' \citep{wang2020mitigating}. This is simply inaccurate (check how many were available at the time), however researchers may not be aware due to sparsity. 

``For dataset consumers, the primary objective is to ensure they have the information they need to make informed decisions about using a dataset. Transparency on the part of dataset creators is necessary for dataset consumers to be sufficiently well informed that they can select appropriate datasets for their tasks and avoid unintentional misuse.'' \citep{gebru2018datasheets}

Centralissimo \citet{muller2019how} con discovery, capture, curation, design, creation.

Centralissimi anche \citet{bao2021COMPASlicated,paullada2020data,crawford2021excavating}. Su privacy (anonymization e consent) pure \citet{wieringa2021data}.



\afabcomment{For intro: define fairness as equalization or lack of bias and bias as non-equality, poppulations/groups. Define both individual and group fairness.}

\afabcomment{Ecco, il cappello è tipo 1) Sta roba è importante e la gente se ne sta accorgendo. 2) Un problema fondamentale è che manca documentazione 3) Un problema da gestire è opacity (compilare info per uno specifico dataset) 4) Un altro problema è scatteredness (forse meglio sparsity), cioè che le info esistono un po' qui e un po' lì. Anche il semplice sapere che un dataset esiste non è banale 5) opacity+scatteredness=documentation debt. Lì attacchi descrivendo i nostri contributi per ridurre il documentatoin debt, cioè la di documentazione in larghezza e quello in profondità, che assembla informazioni da fonti disparate in unico lavoro. Spiega un po' in che modo può essere utile e che da entrambi si posso trarre delle insight di alto livello sui dataset da diversi punti di vista}



\section{Motivazione e Prior Art}
\begin{itemize}
    \item \citet{bender2021dangers} \afabcomment{Uno dei paper più chiacchierati del 2021} borrow the expression \textbf{\emph{documentation debt}} from code development to discuss reliance on datasets that are not properly documented. \afabcomment{L'idea è che se dai in pasto al tuo modello dati di cui sai poco o nulla otterrai degli output parimenti imprevedibili, il che è la radice di tantissimi problemi di bias nei modelli}. \emph{Documentation debt} is central to our work, which goes a long way towards reducing this debt for the FAccT community. As an example,  \citet{bandy2021addressing} and \citet{garbin2021structured} are two works from May 2021 that produce datasheets for one dataset each and that's their only contribution. We provide 3 dasheets+nutritional\_labels for the most popular datasets in the FAccT community and hundreds of data briefs.
    \item  Un altro mega-assist motivazionale per questo lavoro ce lo fornisce Moritz Hardt (uno dei papà della fairness) nel suo intervento al workshop ELLIS di magio 2021, dove fa una preview di un suo lavoro ongoing \url{https://www.youtube.com/watch?v=OZtuVKWqhl0}. Nel video, da 5.37.00, mette in luce un'importantissima contraddizione della comunità FAccT, che da un lato  presta molta attenzione a temi di qualità e trasparenza dei dataset, dall'altro usa tantissimo un dataset (Adult) che ha tutta una serie di problemi, sia di trasparenza che di qualità.
    \item \citet{paullada2020data} survey issues in dataset design and development.  They emphasize the importance of selection,  collection, annotation, documentation, privacy. These are all aspects we consider in our data briefs.
    \item \citet{geiger2020garbage} study the issue of transparency in documenting the provenance of human labels (ground truths annotated by humans). This is another aspects we pay attention to in our data briefs, especially when it comes to the provenance of sensitive attributes.
    \item \citet{jo2020lessons} emphasize the importance of mission statement for dataset documentation. This is another aspect we pay attention to in our data brief description field.
    \item \citet{ekstrand2018privacy} discuss the importance of privacy for individuals whose data is contained in datasets and highlight deanonymization risks. We treat identity as one of the sensitive attributes in our data briefs, highlighting datasets where reidentification seems rather easy (e.g. when names are available).
    \item ArXiv will start linking to dataset.\footnote{\url{https://medium.com/paperswithcode/datasets-on-arxiv-1a5a8f7bd104}} UCI has a new beta version with more emphasis on documentation.\footnote{\url{https://archive-beta.ics.uci.edu/}} This is a sign of increased attention to datasets in the ML community. 
    \item Un'altra iniziativa recente (Google) sulla documentazione dei dataset \url{https://pair-code.github.io/datacardsplaybook/}.
    \item Also a NeurIPS track dedicated to datasets is starting in 2021 \url{https://neuripsconf.medium.com/announcing-the-neurips-2021-datasets-and-benchmarks-track-644e27c1e66c}
    \item \citet{gebru2018datasheets} propose datasheets for datasets as a tool to increase transparency, mitigate biases and help practitioners and researchers select approprate datasets for their task. \afabcomment{Datasheet, che noi adottiamo}
    \item \citet{holland2018dataset} propose a coincise approach, more focused on quantitative results. \afabcomment{Nutritional labels, che noi adottiamo}.
    \item \citet{bender2018data} propose data stements, a documentation framework specific to NLP.
    \item \citet{miceli2021documenting} discuss the importance of documentation in computer scienceand survey issues that hinder the documentation of image datasets.
    \item \cite{denton2020bringing}.
    \item \url{https://arxiv.org/abs/2012.15816}
\end{itemize}


\section{Datasheet and Nutritional Labels}

Un primo contributo del nostro lavoro è documentare i 3 dataset più popolari nel mondo fairness in profondità, compilandone retroattivamente sia il datasheet \citep{gebru2018datasheets} che la nutritional label \citep{holland2018dataset}. In questa sezione riporteremo solo Adult per brevità, ma abbiamo anche gli altri due in uno stato simile, completi ma da rivedere.

\textbf{Key insight} legati a questi 3 dataset (Adult, COMPAS e German)
\begin{itemize}
    \item Sono tutti e tre rumorosi da molti punti di vista. La pulizia del dato non è certo il loro forte e questo emerge in modi diversi nei tre. A riguardo \citet{gromping2019:sg} ha fatto un intero report per correggere degli errori veramente grossolani del German e si è presa la briga di rilasciarne una versione ripulita. Ad oggi, a distanza di 2 anni il suo report ha 3 citazioni sicché darle visibilità mi pare molto utile. Adult è un campione di dati del censimento US 1994 un po' arbitrari, contiene variabili ridondanti e una che nessuno ha mai capito veramente cosa sia. COMPAS è un macello, nonostante gli eccellenti sforzi di Propublica che quella volta lo ha assemblato incrociando dati da 3 fonti diverse. E' pieno di variabili ridondanti. Non si sa veramente chi sia stato rilasciato e chi no, i ricercatori devono decidere in maniera un po' arbitraria sulla base delle date di arresto e rilascio. La procedura di selezione dei dati da includere non è stata uniforme fra  i recidivi e i non recidivi \citep{barenstein2019propublica}.
    \item Due su tre sono vecchi. Adult del 1994, German del $\sim$1975.
    \item Rich get richer. A meno che uno non abbia in mente una specifica applicazione di risk assessment per sistema giudiziario (nel qual caso ci sta che usi COMPAS), esistono dei dataset più rilevanti ed appropriati. Tuttavia, questi tre dataset sono diventati degli standard de-facto nella counità su cui testare i propri algorirtmi/approcci. \afabcomment{A riguardo può essere interessante un grafico a barre di quanto usati sono tutti i $\sim200$ dataset che abbiamo documentato. Il grafico ha una breve testa di $\sim10$ dataset usati in 10+ articoli e una lunghissima coda di roba usata poco.}
\end{itemize}

\textbf{Ulteriori contributi}
\begin{itemize}
    \item I datasheet che abbiamo compilato fungono da riferimento per chi è interessato ad aspetti salienti di questi dataset quali e.g. motivation, composition e collection process.
    \item La nutritional label può fornire delle prime coordinate sulle variabili in gioco, fra cui (fondamentale e spesso più difficile da reperire di quanto si pensi) il loro significato, lo spettro dei valori possibili, i valori più comuni.
\end{itemize}

\textbf{Todos}
\begin{itemize}
    \item Dare una passata ad ogni dataset e sistemare un po' di cosine (vedi e.g. commenti nei datasheet).
    \item Fatto questo, individuare gli aspetti di ogni dataset che ci sembrano più incerti/problematici e contattare i loro creatori per chiarimenti.
\end{itemize}


\FloatBarrier
	
\section{Data briefs}

Un secondo contributo, a mio giudizio anche più importante del primo, è documentare in breve ogni dataset che abbiamo incontrato. Siamo in dirittura d'arrivo, prevedo che arriveremo a poco meno di 200 dataset. A fine sezione ne includo una decina per dare un assaggio.

\textbf{key insight}: Ci sono diverse caratteristiche di un dataset e di come può essere utilizzato in letteratura fairness. Riportiamo di seguito le più interessanti. Ognuna di queste può essere discussa in un'overview generale dei risultati, prima di presentare le data brief di tutti i dataset.
\begin{itemize}
    \item dominio del dataset. Sta emergendo una grande ampiezza di domini in cui si pensa alla fairness. Abbiamo e.g. social networks, finance, computer vision, natural language processing, healthcare, education, marketplaces, labour, criminal justice.
    \item task per cui un dataset è utilizzato. Sta emergendo anche una gran varietà di task in letteratura fairness. Diversi dataset sono usati per diversi task, fra cui: bias discovery, rich-subgroup fair classification, fair ranking, fair sentiment analysis, fair clustering, fair risk assessment, fair representation learning (giusto per menzionarne qualcuno).
    \item attributi sensibili. Per ogni dataset documentiamo quali sono. Di solito c'è un'elevata attenzione agli attributi sensibili (come ci si aspetterebbe da questa comunità). In alcuni casi però gli attributi sensibili sono assenti (vedi punto successivo), oppure un po' buttati là (e.g. RFW chiama race una cosa che può avere come valori Asian, Indian, Caucasian, African) o non è chiaro come vengono ottenuti, e.g. self-reported o etichettati su AMT o etichettati tramite algoritmo. A riguardo la prima è sempre preferibile, le rimanenti sono abbastanza frowned-upon dalla comunità. Ci sono anche attributi protetti domain-specific. \afabcomment{Possibili tag: none, self-reported, labelled by expert, labelled by non-expert, labelled by algorithm and validated, labelled by algorithm, not validated.}
    \item rilevanza sociale dei dataset. Se uno fa ricerca in ambito fairness, presumibilmente ci tiene ad usare dataset che rappresentano fenomeni sociali importanti, o che quantomeno contentogno umani. Esistono però anche parecchi dataset utilizzati nella comunità e da noi documentati che sembrano avere poco a che fare con l'equità degli algoritmi. Per esempio, molti lavori che si occupano di fair representation learning utilizzano dataset artificiali di computer vision in cui non c'è nessun essere umano e nessun reale attributo protetto. Con questo non vogliamo affossarli, ci sono buone ragioni per usare dataset artificiali in questo ambito ma è sicuramente possibile avere anche dei dataset ``reali''. \afabcomment{Possibili tag: highly relevant, mostly irrelevant. Mi limiterei ad una discussione binaria}
    \item Attention to re-identification. Anche la privacy degli individui è importante. Ci sono dei dataset costruiti secondo questo principio (e.g. RtGender) con tecniche di anonimizzazione, altri prestano poca attenzione al tema, anzi rendono disponibili nomi e cognomi delle persone (COMPAS).  \afabcomment{Possibili tag: straightforward identification (requires zero effort, names and last names are avilable), plausible re-identification (e.g. from twitter handles), hard re-identification (e.g. substitution of facebook id with randomized id)}
    \item diversi ruoli dei dataset. A seconda di come viene usato un dataset, questo può avere 6 ruoli diversi \citep{barocas2019fair}, Chapter 7.\footnote{Also discussed in AIES 2021 keynote \url{https://www.aies-conference.com/2021/keynote-speakers/}} Nel documentare questi dataset li troviamo tutti o quasi. I ruoli sono (1) A real world source of data (did not just make up / cherry-picked data) \afabcomment{Some are obvious and connected with attention to social relevance and protected attributes (e.g. Iris, MNIST). Arguably, also datasets that are not really connected to a relevant task, such as Adult, may often fall in this category.}; (2) Spur algorithmic insight and bring about domain-specific progress (resources catalyze attention, e.g. COMPAS) (3) Enable tracking progress over time (come imagenet con CV); (4) Enable model comparison, stile leaderboard, per decidere se un approccio è più efficace di un altro. (Questo probabilmente è il meno presente in letteratura fairness perché si fa fatica a condordare il criterio di fairness più rilevante, di conseguenza c'è poco da comparare non avendo un consenso su cosa misurare. Almeno un esempio di utilizzo in questa direzione mi viene in mente \citep{friedler2019comparative}); \afabcomment{\citet{barocas2019fair} merge (2)--(4) into ``A catalyst and measure of domain-specific progress''. Un esempio in senso lato è COMPAS. sicuramente un catalyst e casestudy per la ricerca di algorithmic fairness. Un esempio in senso più stretto è Jigsaw Unintended Bias in Toxicity Classification challenge (strinctly a domain) o winogender/winobisa (more of a task), che sono più legati al punto (2), mentre Adult, RIcci e gli altri usati in \citet{friedler2019comparative} sono più allineati al punto (3).} (5) source of pretraining data \afabcomment{e.g. i dataset su cui vengono allenati language models ed embeddings -- vedi Wikipedia Dumps}; (6) source of training data (un esempio perfetto è \citet{babaeianjelodar2020quantifying}). A questi sei utilizzi, in letteratura fairness si aggiunge (7) bias audit del dataset (per capire e.g. se va bene come benchmark per un audit o mettere in relazione i suoi bias con quelli presenti nei modelli che lo usano come training set) (8) audit of specific service/product \cite{dash2021when}, simile ad hypothesis testing in medical trials. Da un lato, probabilmente il (7) può essere indirettamente re-inquadrato nei sei di Arvind, nel senso che uno fa un audit di un dataset non per il gusto di farlo ma perché ha in mente che quel dataset ha una rilevanza come risorsa per il training o la misura. Dall'altro, dataset tipo quello di Safegraph \citep{coston2021leveraging} vengono usati per informare decisioni di public policy, e si meritano degli audit a prescindere da potenziali utilizzi ML-osi.
    \item Attention to consent. MS-Celeb-1M is a fairly egregious example, while the Chicago Face Database had a clear consent procedure (`` Upon arrival, participants were asked to carefully read a consent/release form, allowing us to use their photos for research purposes''). \afabcomment{Binary discussion?}
    \item Transparency. Clear documentation and clean data. COMPAS \afabcomment{also German} is a negative example here; in its released version it is simply unusable and researchers need to take often undocumented preprocessing steps) \afabcomment{I guess the dataset was simply not released with this intention}. Responsiblity here does not rest solely on the shoulders of those creating and maintaining a dataset. Ad-hoc works may specifically target a documentation debt \cite{gromping2019:sg,bandy2021addressing}; alternatively research works utilizing one such dataset may take some paragraphs to describe preprocessing with enough detail \citep{mishler2021fairness}. These imprecisions may lead to some experimental results which would not otherwise hold, or to lack of reproducibility due to undocumented subjective choices by researchers.  \afabcomment{What is a positive example of a well-documented and clean dataset here?} \afabcomment{Possibili tag: poorly documented dataset, well-documented after a certain point, well-documented since release}
    
    Related to articles, there is article clarity on which dataset is being used. This is often high, however there are occasional situations for which finding the mentioned dataset becomes really hard. One such example is \citep{li2021on} with PubMed, despite providing a direct link to a website, it was easier to find the information by googling. In a few occasions we failed altogether despite the presence of a summary in the article (\citet{noriegacampero2019active} with the mexican household survey). This is more of an article things rather than a dataset thing.
    
    \item Inclusivity. Attention to subpopulation balance (e.g. Adience vs PPB). \afabcomment{Possibili tag: balanced/imbalanced}
\end{itemize}

\textbf{ulteriori contributi}
\begin{itemize}
    \item Le data brief dei dataset fungono da documentazione minima degli stessi, riportando diverse informazioni salienti. Auspicabilmente possono essere utili a ricercatori sia in maniera domain-driven (quali sono i dataset di fairness disponibili in ambito healthcare?) che task-driven (quali sono i dataset di fairness usati per fair clustering?).
\end{itemize}

\textbf{todos}
\begin{itemize}
    \item Complete ``Tasks in fairness literature'' for each dataset. This should be part of the \emph{final pass}, i.e. the last time we go through each article.
    \item Go over and review every data brief.
    \item Improve the ``domain'' field and make it more uniform. For healthcare data, add tags that are more specific.
    \item Sometimes also dataset title can be improved.
\end{itemize}


\section{Note metodologiche}
\subsection{Quali articoli}
\begin{enumerate}
    \item Consideriamo ogni paper pubblicato nei proceedings di  (1) conferenze di settore (FAccT, AIES) (2) gli events (Past Network Events and Older Workshops and Events) del network FAccT listati qui \url{https://facctconference.org/network/} (3) 5 prestigious conferences focused on artificial intelligence, machine learning and data science (CVPR, NeurIPS, ICML, ICLR, KDD) \afabcomment{Qui ovviamente si potrebbe considerare anche altro ma aggiungerebbe poco. Il lavoro starebbe in piedi anche con solo i punti (1) e (2); il (3) è un nice-to-have e a una certa bisogna fermarsi}. Consideriamo solo workshop/conferenze dal 2014 in poi, il primo anno in cui c'è stato un evento dedicato (FAT/ML a NeurIPS). Per ora ci siamo fermati a venue per le quali le decisioni accept/reject e gli articoli accettati erano disponibili entro la prima settimana di maggio 2021.
    \item All'interno di questi proceedings, consideriamo tutti gli articoli contententi nel titolo parole chiave riconducibili alla fairness:
    \begin{itemize}
        \item *fair* (fairness, unfair)
        \item *bias* (biased, debiasing)
        \item discriminat* (discrimination)
        \item *equal* (equality, unequal)
        \item *equit* (equity)
        \item disparate (disparate impact)
        \item *parit* (parity, disparity)
    \end{itemize}
    \item Analizziamo questi articoli e li scartiamo se usano queste parole chiave con significato diverso da quello inteso qui e tipico della comunità FAccT. \afabcomment{Da decidere come parlare di roba tipo \citep{martin2021spoken}, per i quali per il momento abbiamo ricercato i pdf dei lavori pubblicati altrove.} In questo lavoro, \emph{fairness} ha a che vedere con nozioni di giustizia ed equità, che calate in ambito algoritmico si traducono spesso con l'idea di equalizzare qualche metrica per diverse classi demografiche o individui (esistono anche eccezioni tipo fairness-through-unawareness che rimangono in scope per questo lavoro in quanto legate a un'idea di giustizia). Invece la parola bias (esempio) può benissimo essere usata in senso statistico (vedi position bias in IR), e legata ad obiettivi di generico miglioramento delle performance, senza avere in mente nozioni di giustizia e gruppi protetti. Articoli di questo tipo (parole chiave giuste, accezione sbagliata) vengono scartati.
    \item Il nostro principio guida è fare del nostro meglio nel documentare. Se il sito di un workshop risulta irraggungibile viene ignorato (successo per un paio di workshop). Idem per i singoli articoli. Per articoli workshop presentati poi a conferenze (stesso titolo) utilizziamo la versione da conferenza per le nostre analisi, considerata più completa. 

\end{enumerate}

\subsection{Quali dataset:}
\begin{enumerate}
    \item Ad ogni articolo che passa questa scrematura, associamo i dataset rilevanti al suo interno (if any). Un dataset è rilevante per un articolo se (1) viene utilizzato come risorsa per allenare o valutare algoritmi, (2) se l'articolo effettua un'analisi (audit) del dataset in questione o (3) se l'articolo presenta un unovo dataset.
    \item Assegnamo ai dataset reperiti un ID e ne incrementiamo il contatore ad ogni articolo associato.
    \item Produciamo una data brief per tutti i dataset che rispettano uno dei seguenti criteri di inclusione:
    \begin{itemize}
        \item in any of the papers associated with the dataset or respective code repositories we find a working link, reference (citation) or a name which leads to hits on a search engine, and, upon deeper inspection, the documentation we find for the dataset does not contradict the information provided in the paper (segno che il dataset usato non è quello trovato googlando).
        \item in any of the papers associated with the dataset there is enough information for said paper to become a primary source of information on the dataset. This is typically the case for articles presenting a novel dataset.
    \end{itemize}
    Succede di rado (su dataset sfigati) che nessuna delle condizioni sopra sia vera. Un esempio è il dataset denominato \emph{Sentencing} in \citet{berk2017convex}. Ovviamente, tanto più un dataset è utilizzato in letteratura fairness, tanto meno è probabile che succeda.
    
    Escludiamo poi due tipologie di risorse ``borderline'':
    \begin{itemize}
        \item we omit datasets that are only used as minor sources of auxiliary information, e.g. to know the percentage of US residents in each state.
        \item we do not consider Word Embeddings as datasets. We only consider the corpora they are trained on if WEs are trained and not taken off-the-shelf. 
        \item we omit user studies/surveys unless we find them to be used in articles other than the one introducing it (examples: Crowd judgement, Willingness-to-Pay for Vaccine), taking this as a sign that the data from the survey produced a data artifact with some users. \afabcomment{probably redundant if we omit (3) se l'articolo presenta un nuovo dataset}
        \item we omit toy datasets unless we find them to be used in more than one article (examples: toy datasets1-4).
    \end{itemize}
\end{enumerate}

\section{Conclusion}
Read conclusion of \citet{geiger2020garbage}.

\clearpage


==> sections/2022_update.tex <==
\section{2022 Updates}
\afabcomment{Do not include}

calendar of conf:
\begin{itemize}
    \item FAccT: March 2021, May 2022
    \item ICLR: May 2021, Apr 2022
    \item AIES: May 2021, August 2022
    \item CVPR: June 2021, June 2022
    \item ICML: Jul 2021, Jul 2022
    \item KDD: Aug 2021, Aug 2022
    \item EAAMO: Oct 2021, Oct 2022
    \item NeurIPS: Dec 2021, Dec 2022
\end{itemize}

Keywords:
\begin{itemize}
    \item fair
    \item bias
    \item discriminat
    \item equal
    \item equit
    \item parit
    \item disparate
\end{itemize}

\section{AIES 21}:

\url{https://dl.acm.org/doi/proceedings/10.1145/3461702}

\begin{itemize}
    \item \citet{cooper2021emergent} none.
    \item \citet{dai2021fair} toy dataset.
    \item \citet{diana2021minimax} Communities and Crime [fair regression], COMPAS [fair classification], Bank Marketing [fair classification], Seoul Bike Sharing (NEW) [fair regression], Internet Traffic (prob KDD Cup 99, not enough info).
    \item \citet{fish2021reflexive} none
    \item \citet{kasirzadeh2021fairness} none
    \item \citet{shekhar2021fairod} Adult [fair anomaly detection], Credit Card Default [fair anomaly detection], Internet Ads [fair anomaly detection] (\url{https://archive.ics.uci.edu/ml/datasets/internet+advertisements}) (NEW)
    \item \citet{tomasev2021fairness} none.
    \item \citet{bakker2021beyond} Adult [fair active classification]. 
    \item \citet{belitz2021automating} Student [Fair data summarization], Student academics [Fair data summarization] (NEW), Adult [Fair data summarization]
    \item \citet{biswas2021ensuring} COMPAS [Robust fair classication], MEPS-HC [Robust fair classication]
    \item \citet{castro2021fairness} none
    \item \citet{fabris2021algorithmic} RCA [Fairness pricing evaluation] (NEW)
    \item \citet{fleisher2021what} none
    \item \citet{galhotra2021learning} Adult [Preference-based fair clustering], Bank Marketing [Preference-based fair clustering], Communities and Crime [Preference-based fair clustering].
    \item \citet{hannan2021who} none
    \item \citet{islam2021can} COMPAS [Fairness evaluation], Adult [Fairness evaluation], Bank Marketing [Fairness evaluation], Heritage Health [Fairness evaluation] 
    \item \citet{jiang2021towards} Berkeley Students [Fair classification] (NEW)
    \item \citet{kuhlman2021measuring} NFL rankings [Fair Ranking Evaluation] (NEW)
    \item \citet{liu2021rawlsnet} IBM HR (synthetic) (NEW) [Fair data generation], Campus recruitment [Fair  data generation] (NEW)
    \item \citet{loi2021fair} none
    \item \citet{mazijin2021how} none
    \item \citet{mhasawade2021causal} Adult [Fair classification]
    \item \citet{perrier2021quantum} none
    \item \citet{perrone2021fair} Adult [Fair classification], German Credit [Fair classification], COMPAS [Fair classification]
    \item \citet{prost2021measuring} none
    \item \citet{schumann2021step} Open Images Dataset [Data bias evaluation] (NEW)
    \item \citet{segal2021fairness} UTK Face, Labeled Faces in the Wild, Color MNIST, CelebA, Adult, Timit (NEW) [Fairness evaluation]
    \item \citet{shah2021rawslian} Wikipedia Toxic Comments, Adult, Bank Marketing [Fair classification]
    \item \citet{sharma2021fairn}  Adult, German Credit, MEPS-HC [Fair classification]
    \item \citet{suhr2021does} Task Rabbit (NEW) [Fair ranking evaluation] (although it's more of multi-stage fairness evaluation)
    \item \citet{yaghini2021human} none
    \item \citet{chen2021gender} Wikipedia Dumps [Bias evaluation in WEs] (NEW variant, done)
    \item \citet{guo2021detecting} WEAT [Bias Evaluation in Language Models], Reddit comments 2014 [Bias Evaluation in Language Models] (NEW)
    \item \citet{keswani2021towards} Twitter Offensive Language [Fair multi-stage classification]
    \item \citet{abid2021persistent} none
    \item \citet{aka2021measuring} Open Images Dataset [Fairness Evaluation]
    \item \citet{kasirzadeh2021ethical} none
    \item \citet{kim2021age} FACES [Fairness evaluation of emotion detection] (NEW) \afabcomment{TODO!}
    \item \citet{lee2021risk} none
    \item \citet{pandey2021disparate} Chicago ridehailing data (NEW) [Fairness pricing evaluation]
    \item \citet{ali2021accounting} COMPAS, Stop, Question and Frisk [Fair classification]
    \item \citet{simons2021machine} none
    \item \citet{solans2021comparing} Barcelona real estate [Fair ranking?] (NEW)
    \item \citet{ramachandran2021gaea} University Facebook Networks (NEW variant, done), School Access in Chicago (NEW) [Fair graph mining?]
\end{itemize}

TODOs

\afabcomment{Change noisy if not too burdensome? \emph{under unawareness} should be one subcategory, the other could be related to encryption?} DONE

\afabcomment{Look into 2021, evaluate whether indeed 2021 or present} DONE

\afabcomment{Add fair data generation} DONE

\afabcomment{Update domain, task, role, and data curation themes (anonymization, consent, inclusivity, labeling of sensitive attributes, and transparency)}  DONE

\afabcomment{Add discussion of management information systems under economics and business} DONE

\afabcomment{Update data briefs with tasks from non-new datasets.}  DONE

\afabcomment{FACES [Fairness evaluation of emotion detection] (NEW) } DONE

\afabcomment{New present vs 2021 } DONE

\afabcomment{Address afabcomments laying around main text.} DONE


\afabcomment{Wink at EAAMO} DONE


\afabcomment{Fix refs to DCAT in appendix} DONE


\afabcomment{Send to creators}. DONE

\afabcomment{Update figures, tables and appendix via python}. DONE

\afabcomment{Update main text to reflect new conference coverage and rough number of articles} DONE

\afabcomment{Update precise figures on dataset usage in main text} DONE

\afabcomment{Summary table with domain, subdomain, subsubdomain} DONE

\afabcomment{proof read}

\section{CVPR 2021}

\url{https://openaccess.thecvf.com/CVPR2021?day=all}

\begin{itemize}
    \item \citet{ramaswamy2021fair} CelebA [fair data generation]
    \item \citet{jung2021fair} UTKFace, CelebA, CIFAR10S (NEW variant) [fair classification]
    \item \citet{xu2021consistent} BUPTFace [fair classification]
    \item \citet{gong2021mitigating} RFW, BUPT [fair representation learning]
\end{itemize}

\section{ICML 2021}

\url{https://proceedings.mlr.press/v139/}

\begin{itemize}
    \item \citet{balseiro2021regularized} Display advertisement (NEW) [fair resource allocation]
    \item \citet{celis2021fair} Adult, COMPAS [fair classification under unawareness] 
    \item \citet{correa2021fairness} Bank Marketing [fair classification]
    \item \citet{coston2021characterizing}  COMPAS, Commonwealth Bank of Australia (NEW) [fair classification]
    \item \citet{gorantla2021on} German credit, COMPAS [Fair ranking].
    \item \citet{jalal2021fairness}.  MNIST, Flickr Faces (NEW), cats and dogs (NEW)  [fair super resolution]
    \item \citet{lee2021fair}. Adult, CelebA, Civil Comments, and CheXpert [Fair selective classification]
    \item \citet{li2021fair} Vehicle, FEMNIST (NEW), CelebA, Fashion MNIST, StackOverflow (NEW) [fair robust federated learning].
    \item \citet{}.
    \item \citet{}.
    \item \citet{}.
    \item \citet{}.
    \item \citet{}.
\end{itemize}



%I am the true template, copy me
\subsection{Template}
\begin{itemize}
    \item \textbf{Description}: 
    \item \textbf{Affiliation of creators}: 
    \item \textbf{Domain}: 
    \item \textbf{Tasks in fairness literature}: 
    \item \textbf{Data spec}: 
    \item \textbf{Sample size}: 
    \item \textbf{Year}: 
    \item \textbf{Sensitive features}: 
    \item \textbf{Link}: 
    \item \textbf{Further info}: 
    \item \textbf{Contact1}: 
    \item \textbf{Email1}: 
    \item \textbf{Contact2}: 
    \item \textbf{Email2}: 
\end{itemize}


==> sections/abstract_c.tex <==
A growing community of researchers has been investigating the equity of algorithms, advancing the understanding of risks and opportunities of automated decision-making for historically disadvantaged populations. Progress in fair Machine Learning (ML) hinges on data, which can be appropriately used only if adequately documented. Unfortunately, the research community, as a whole, suffers from a collective data documentation debt caused by a lack of information on specific resources (\emph{opacity}) and scatteredness of available information (\emph{sparsity}). In this work, we survey over two hundred datasets employed in algorithmic fairness research, producing standardized and searchable documentation for each of them. Moreover we rigorously identify the three most popular fairness datasets, namely Adult, COMPAS, and German Credit, for which we compile in-depth documentation. This unifying documentation effort targets \emph{documentation sparsity} and supports multiple contributions. In the first part of this work, we summarize the merits and limitations of Adult, COMPAS, and German Credit, adding to and unifying recent scholarship, calling into question their suitability as general-purpose fairness benchmarks. To overcome this limitation, we document hundreds of available alternatives, annotating their domain and the algorithmic fairness tasks they support, along with additional properties of interest for fairness practitioners and researchers, including their format, cardinality, and the sensitive attributes they encode.  In the second part, we summarize this information, zooming in on the domains and tasks supported by these resources. Overall, we assemble and summarize sparse information on hundreds of datasets into a single resource, which we make available to the community, with the aim  of tackling the data documentation debt.

%and aim to update on a yearly basis.

==> sections/conclusions_c.tex <==



\section{Conclusions }
\label{sec:conclusion}
Algorithmic fairness is a young research area, undergoing a fast expansion, with diverse contributions in terms of methodology and applications. Progress in the field hinges on different resources, including, very prominently, datasets. In this work, we have surveyed hundreds of datasets used in the fair ML and algorithmic equity literature to help the research community reduce its documentation debt, identify gaps, and improve the utilization of existing resources. 
%We have shown two different phenomena at work hindering an optimal utilization of fairness datasets. Documentation opacity is 

We have rigorously identified the most popular datasets in the literature, and carried out a thorough documentation effort for Adult, COMPAS and German Credit. Our work unifies and adds to recent literature on data studies, calling into question their current status of general-purpose fairness benchmarks, due to contrived prediction tasks, noisy data, severe coding mistakes, limitations in encoding sensitive attributes, and age. In a practical demonstration of documentation debt and its consequences, we find several works of algorithmic fairness using German Credit with sex as a protected attribute, while careful analysis of recent documentation shows that this feature cannot be reliably retrieved from the data.

We have documented over two hundred datasets to provide viable alternatives, annotating their domain and the tasks they support in works of algorithmic fairness. We have shown that the processes generating the data belong to many different domains, including, for instance, criminal justice, education, search engines, online marketplaces, emergency response, social media, medicine, hiring, and finance. At the same time, we have described a variety of tasks studied on these resources, ranging from generic, such as \emph{fair  regression}, to  narrow such as \emph{fair districting} and \emph{fair truth discovery}. Overall, such diversity of domains and tasks provides a glimpse into the variety of human activities and applications that can be impacted by automated decision making, and that can benefit from fair ML and algorithmic equity research. 

Dataset tasks, domains, and the whole metadata are made available in our data briefs (Appendix \ref{sec:databriefs}), which we plan to update on a yearly basis.\footnote{We aim to release a web app for dataset search at \url{https://fairnessdatasets.dei.unipd.it/}. \label{fn:web_app}} We envision several benefits for the algorithmic equity and data studies research communities, including (1) informing the choice of datasets for experimental evaluations of fair algorithms, including domain-oriented and task-oriented search, (2) directing studies of data bias, and other quantitative and qualitative analyses, including retrospective documentation efforts, towards popular (or otherwise important) resources, (3) identifying areas and sub-problems that are understudied in the algorithmic fairness literature, and (4) supporting multi-dataset studies, focused on resources united by a common characteristic, such as encoding a given sensitive attribute \citep{scheuerman2020how},  concerning computer vision \citep{fabbrizzi2021survey}, or being popular in the fairness literature \citep{lequysurvey2022}.


In this work, we have targeted the collective documentation debt of the algorithmic fairness community, resulting from the opacity surrounding certain resources and the sparsity of existing documentation. We have mainly targeted sparsity in a centralized documentation effort. Similarly to other types of data interventions, useful documentation can be produced after release, but, as shown in this work, the documentation debt may propagate nonetheless. In a mature research community, curators, users and reviewers can all contribute to cultivating a data documentation culture and keep the overall documentation debt in check.

==> sections/intro_c.tex <==

\section{Introduction}

%Following the widespread study and application of data-driven algorithms in contexts that are central to people's well-being, a large community of researchers has coalesced around the growing field of algorithmic fairness and equity, investigating algorithms through the lens of justice, bias, power, harms, and equality. A line of work gaining traction in the field, intersecting with critical data studies, human-computer interaction, and computer-supported cooperative work, focuses on  data transparency and standardized documentation processes to describe key characteristics of datasets \citep{gebru2018datasheets,holland2018dataset,bender2018data,geiger2020garbage,jo2020lessons,miceli2021documenting}. Most prominently, \citet{gebru2018datasheets} and \citet{holland2018dataset} proposed two complementary documentation frameworks, called \emph{Datasheets for Datasets} and \emph{Dataset Nutrition Labels}, to improve data curation practices and favour more informed data selection and utilization for dataset users. Overall, this line of work has contributed to an unprecedented attention to dataset documentation in ML, including a novel track focused on datasets at the Conference on Neural Information Processing Systems (NeurIPS), an initiative to support dataset tracking in repositories for scholarly articles,\footnote{\url{https://medium.com/paperswithcode/datasets-on-arxiv-1a5a8f7bd104}} and dedicated works producing retrospective documentation for existing datasets \citep{bandy2021addressing,garbin2021structured}, auditing their properties \citep{prabhu2020large} and tracing their usage \citep{peng2021mitigating}.

Data documentation is important and caters to different goals. It increases transparency, favouring an improved understanding of the data and resulting models \citep{hutchinson2021towards}, it reduces chances of data misuse \citep{gebru2018datasheets} and supports accountability in dataset and model creation \citep{hutchinson2021towards}, it helps connect the data with its context to guide scientific inquiry \citep{paullada2020data}, and it makes the values influencing dataset curation explicit \citep{scheuerman2021datasets}. In the field of software development, technical debt is a cost incurred when speed of execution is prioritized over quality \citep{hutchinson2021towards}. In recent work, \citet{bender2021:dangers} propose the notion of \emph{documentation debt}, in relation to training sets that are undocumented and too large to document retrospectively. This debt compounds over time, with serious consequences on dataset understanding and use. We extend this definition to the collection of datasets employed in a given field of research. We see two components at work contributing to the documentation debt of a research community. On one hand, \emph{opacity} is the result of poor documentation affecting single datasets, contributing to misunderstandings and misuse of specific resources. On the other hand, when relevant information exists but does not reach interested parties, there is a problem of documentation \emph{sparsity}. One example that is particularly relevant for the algorithmic fairness community is represented by the German Credit dataset \citep{hofmann1994:sg}, a popular resource in this field. Many works of algorithmic fairness, including recent ones, carry out experiments on this dataset using sex as a protected attribute \citep{he2020geometric,yang2020fairness,baharlouei2020renyi,lohaus2020too,martinez2020minimax,wang2021fair,perrone2021fair,sharma2021fairn}, while existing yet overlooked documentation shows that this feature cannot be reliably retrieved \citep{gromping2019:sg}.\footnote{Hereafter, for brevity, we only report dataset names. The relevant references and additional information can be found in Appendix \ref{sec:databriefs}.} %Moreover, the mere fact that a dataset exists and is relevant to a given task or a given domain may be unknown. The BUPT Faces datasets, for instance, were presented as the second existing resource for face analysis with race annotations \citep{wang2020mitigating}. However several resources were already available at the time, including Labeled Faces in the Wild \citep{han2014age}, UTK Face \citep{zhifei2017age}, Racial Faces in the Wild \citep{wang2019racial}, and Diversity in Faces \citep{merler2019diversity}.

To tackle the documentation debt of the algorithmic fairness community, we survey the datasets used in over 500 articles on fair ML and equitable algorithms, presented at seven major conferences, considering each edition in the period 2014--2021, and more than twenty domain-specific workshops in the same period. We find over 200 datasets employed in studies of algorithmic fairness, for which we produce compact and standardized documentation, called \emph{data briefs}. Data briefs are intended as a lightweight format to document fundamental properties of data artifacts used in algorithmic fairness, including their purpose, their features, with particular attention to sensitive ones, the underlying labeling procedure, and the envisioned ML task, if any.
%Moreover, they report the affiliation of creators, year, data format, sample size, and sensitive features. 
To favor domain-based and task-based search from dataset users, data briefs also indicate the domain of the processes that produced the data (e.g., radiology) and list the fairness tasks studied on a given dataset (e.g. fair ranking). For this endeavour, we have contacted creators and knowledgeable practitioners identified as primary points of contact for the datasets. We received feedback (incorporated into the final version of the data briefs)
%on preliminary versions of the data briefs 
from 79 curators and practitioners, whose contribution is acknowledged at the end of this article. Moreover, we identify and carefully analyze the three datasets most often utilized in the surveyed articles (Adult, COMPAS, and German Credit), retrospectively producing a \emph{datasheet} \citep{gebru2018datasheets} and a \emph{nutrition label} \citep{holland2018dataset} for each of them. From these documentation efforts, we extract a summary of the merits and limitations of popular algorithmic fairness benchmarks, and a categorization of alternative resources with respect to domains and tasks in works of algorithmic fairness.
Overall, we make the following contributions.
\begin{itemize}
    \item \textbf{Unified analysis of popular fairness benchmarks}. We produce datasheets and nutrition labels for Adult, COMPAS, and German Credit, from which we extract a summary of their merits and limitations. We add to and unify recent scholarship on these datasets, calling into question their suitability as general-purpose fairness benchmarks due to contrived prediction tasks, noisy data, severe coding mistakes, limitations in encoding sensitive attributes, and age. Table \ref{tab:popular} summarizes this contribution.
    \item \textbf{Survey of existing alternatives}.  We compile standardized and compact documentation for over two hundred resources used in fair ML research, annotating their domain and the tasks they support in works of algorithmic fairness. By assembling sparse information on hundreds of datasets into a single document, we aim to support multiple goals by researchers and practitioners, including domain-oriented and task-oriented search by dataset users. Contextually, we provide a novel taxonomy of tasks and domains investigated in algorithmic fairness research (summarized in Tables \ref{tab:taskwise} and \ref{tab:domainwise}).
\end{itemize}

\noindent \textbf{Roadmap}. Readers looking for alternative fairness datasets should prioritize Section \ref{sec:alternatives}, Appendix \ref{sec:databriefs}, and take account of the web app under development (see Footnote \ref{fn:web_app}). Overall, this work is organized as follows. Section \ref{sec:related} introduces related works. Section \ref{sec:methodology} presents the methodology and inclusion criteria of this survey. Section \ref{sec:popular} analyzes the perks and limitations of the most popular datasets. Section \ref{sec:alternatives} discusses alternative fairness resources from the perspective of the underlying domains and supported tasks. Finally, Section \ref{sec:conclusion} contains concluding remarks and details the broader importance of this work for the research community. Interested readers may find the data briefs in Appendix \ref{sec:databriefs}, followed by the detailed documentation produced for Adult, COMPAS, and German Credit.


%horizontal works across multiple data sources
%\begin{itemize}
%    \item \citet{lequysurvey2022} tabular data. 15 datasets. We do not cover KDD census, oulad. They obtain counter-intuitive results on German due coding mistakes. They perform a quantitative analysis of 15 datasets, while listinng their domain, protected attributes, collection period and location.
%    \item \citet{fabbrizzi2021survey}. focus on visual datasets, describing types of bias affecting them, methods for discovering and measuring bias, and summarizing some datasets that were created to measure and tackle bias in computer vision.
%    \item \citet{geiger2020garbage} study the transparency in documentation of labeling practices employed in over 100 datasets about Twitter.
%    \item \citet{leonelli2020data} study practices of collection, cleaning, clustering, visualization, sharing and analysis across a variety of research domains.
%    \item \citet{romei2014multidisciplinary} survey techniques and data for discrimination analysis, used in works that are more focused on evaluation rather than a proposal of novel solutions.
%    \item \citet{peng2021mitigating} identify three popular face and person recognition datasets, and analyze related ethical concerns stemming from derivative datasets and models, lack of clarity of licenses, and dataset management practices.
%    \item \citet{crawford2021excavating} focus on datasets commonly used as training sets in computer vision, from the perspective of associated labels and underlying taxonomies.
%\end{itemize}


%vertical works focusing on a single resource
%\begin{itemize}
    %\item \citet{prabhu2020large} focus on Imagenet (ILSVRC 2012) which they analyze along the lines of consent, problematic ( verifiably pornographic) content, and individual re-identification.
    %\item \citet{kizhner2020digital} study issues of representation in the Google Arts and Culture project across countries, cities and institutions.
    %\item \citet{hardt2021facing} analyze numerical idiosyncrasies in the Adult dataset, and propose a novel version, for which they provide a daasheet.
    %\item \citet{barenstein2019propublica} analyze numerical idiosyncrasies in the COMPAS dataset.
    %\item \citet{bao2021COMPASlicated} sources of bias in COMPAS.
    %\item \citet{gromping2019:sg} German analysis of issues resulting from coding mistakes and novel release.
    %\item \citet{bandy2021addressing} Book Corpus datasheet.
    %\item \citet{garbin2021structured} Chexpert dayasheet.
%\end{itemize}

%documentation frameworks
%\begin{itemize}
%    \item \citet{gebru2018datasheets}
%    \item \citet{holland2018dataset}
%    \item \citet{bender2018data}
%    \item \citet{miceli2021documenting} (more of a broader proposal)
%\end{itemize}


%fairness surveys
%\begin{itemize}
%%    \item \citet{caton2020fairness} methods and measures. Tiny taxonomy (<10)
%    \item \citet{mehrabi2019survey} methods, measure and sources of bias. Contains some tiny taxonomy of tasks.
%    \item \citet{pessach2020algorithmic} methods, measure, sources of bias, datasets (12), tiny taxonomy of tasks (<10).
%    \item \citet{chouldechova2020snapshot} maybe
%\end{itemize}

%domain-specific ones occasionally covering datasets
%\begin{itemize}
%    \item fair ranking \citet{pitoura2021fairness} measures and methods
%    \item fair ranking \citet{zehlike2021fairness} with datasets (19).
%    \item gender bias in NLP \citet{sun2019mitigating} methods
%    \item fairness in computational medicine \citet{xu2022algorithmic}.
%\end{itemize}




